Accurate Models of AMD Matrix Cores

Matrix multipliers available on recent GPUs do not conform with the IEEE 754 floating point standard. Features of matrix multipliers differ across vendors and architectures of the same vendor, such as accumulator width, rounding behaviour, normalisation points, intermediate underflow and overflow logic, the handling of subnormals, and the treatment of special inputs. As a result, reproducibility of small matrix multiplier results across devices is not possible and cannot be achieved by software control. Implementation details of matrix multipliers are not documented, making it difficult to interpret discrepancies in the computed results. We characterise the numerical behaviour of matrix multipliers across three AMD GPU architectures: CDNA 1, CDNA 2, and CDNA 3, using the MI100, MI210/250, and MI300A/300X GPUs, respectively. We design test vectors to target numerical features for all supported input formats and provide the derivation and the reasoning for why each vector allows to determine a particular numerical feature based on the outputs of the devices. MATLAB-based software models of the matrix multipliers are then developed for each architecture and validated for bit-level reproducibility against hardware using a randomized test suite consisting of 10 million sets of random input vectors. To achieve this, we applied a previously developed technique to iteratively refine the accuracy of the models in a loop, by randomized testing followed by test-refinement until the model matches the hardware for every test case. Finally, as a proof of concept for what experimental research can be done with the models, we have utilised them in two demonstrative numerical applications, quantifying application-level accuracy differences between AMD matrix cores and the NVIDIA tensor cores.

==> diagrams/dominant_eigenvalue.tex <==

\begin{figure*}
  \begin{center}
    \footnotesize
    \begin{tikzpicture}
      \begin{groupplot}[
        group style={
          group size=3 by 3,
          vertical sep=1.2cm
        },
        %ymode=log,
        %xmode=log,
        width=1.9in,
        height=1.6in,
        grid=major,
        ymax = 400,
        ymin = 50,
        every axis plot/.append style={mark repeat=4}
        ]

        \nextgroupplot[
        ylabel={$\lambda_{1,1}(\mathrm{e}^{\mathrm{j}\Omega})$},
        align=left,
        title={GEMM fp8-e5m2},
        xlabel = {$\Omega$}
        ]

        \addplot[color=blue!70, mark=x] table [x=Omega, y=lambda] {pevd_data/Gfreq_Reference_11_abs.dat};
        \addplot[color=red!70, mark=o] table [x=Omega, y=lambda] {pevd_data/Gfreq_fp8-e5m2_Ada_11_abs.dat};
        \addplot[color=green!70, mark=o] table [x=Omega, y=lambda] {pevd_data/Gfreq_fp8-e5m2_H100_11_abs.dat};
        \addplot[color=black!70, mark=o] table [x=Omega, y=lambda] {pevd_data/Gfreq_fp8-e5m2_B200_11_abs.dat};
        
        \nextgroupplot[
        align=left,
        title={Quad-word (fp8-e5m2)},
        xlabel = {$n$}
        ]

        \addplot[color=blue!70, mark=x] table [x=n, y=error] {data/matmul_test_fp8-e5m2_binary32_words_4_model_mi300x.dat};
        \addplot[color=red!70, mark=o] table [x=n, y=error] {data/matmul_test_fp8-e5m2_binary32_words_4_model_b200.dat};

        \nextgroupplot[
        align=left,
        title={6-word (fp8-e5m2)},
        xlabel = {$n$}
        ]

        \addplot[color=blue!70, mark=x] table [x=n, y=error] {data/matmul_test_fp8-e5m2_binary32_words_6_model_mi300x.dat};
        \addplot[color=red!70, mark=o] table [x=n, y=error] {data/matmul_test_fp8-e5m2_binary32_words_6_model_b200.dat};

      \end{groupplot}
    \end{tikzpicture}

    \begin{tikzpicture}[trim axis left, trim axis right]
      \begin{axis}[
        title = {},
        legend columns=5,
        scale only axis,
        width=1mm,
        hide axis,
        /tikz/every even column/.append style={column sep=0.4cm},
        legend style={at={(0,0)},anchor=center,draw=none,
          legend cell align={left},cells={line width=0.75pt}},
        legend image post style={sharp plot},
        legend cell align={left},
        every axis plot/.append style={thick}
        ]
        \addplot [color=blue!70, mark=x] (0,0);
        \addplot [red!70, mark=o] (0,0);
        \legend{MI300X, B200};
      \end{axis}
    \end{tikzpicture}
  \end{center}
  \caption{Multi-word arithmetic experiment presented by Mary and Mikaitis~\cite[Sec.~5]{mami25} on the simulation of various tensor cores. We have reproduced the experiment on four different tensor core generations modelled in MATLAB. Relative norm-wise errors of matrix multiplication, compared with a default MATLAB binary64 multiplication, are shown. The input matrices to the GEMM are $A \in R^{10\times n}$ and $B \in R^{n \times 10}$. These matrices are multiplied with a multi-word algorithm \cite[Sec.~4]{mami25} by splitting them into several fp8-e5m2 words.}
   \label{fig:multi-word0}
\end{figure*}


==> sims/feature_table.tex <==
\begin{center}

\rotatebox{90}{%
\begin{minipage}{0.92\textheight}
\centering
\scriptsize

\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.1}

\captionof{table}{Summary of the numerical features of several generations of NVIDIA tensor cores (mixed-precision matrix multipliers) and AMD matrix cores}
\label{tab:nfc}

\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccc}
\toprule
In & GPUs & Prod. Align. & $N_{\mathrm{FMA}}$ & ${c=0}$ & $c$ late/early & \shortstack{$c+s_{p_i-sum}$\\align.} & Final Round & $e^{\mathrm{lim}}_{\mathrm{min}}$ \\
\midrule
%%======================
%% fp8 
%%======================
fp8 & B200 & (2,25) & 32 & discarded & early & - & Trunc. & - \\
& H100 & (2,13) & 32 & discarded & early & - & Trunc. & - \\
& MI300X, MI300A & (2,24) & $8_{\mathrm{odd-even}}$ & subnormal & late & (24,31,RD)* & RNE & - \\
%%====================
%% fp16/bf16
%%====================
fp16/bf16 & H100, B200& (2,25) & 16/16 & discarded &  early & - & Trunc. & -133 \\
& A100 & (2,24) & 8/8 & discarded & early & - & Trunc. & -132 \\
& MI100 & (1,$\infty$) & 4/2 & discarded & early & - & RNE & - \\
& MI300A, MI300X & (2,24) & 8/8 & subnormal & late & (24,31,RD) & RNE & -126 \\
%%===================
%% TensorFloat16
%%===================
tf19 & H100, B200 & (2,25) & 8 & discarded & early & - & Trunc. & -133 \\
& A100 & (2,24) & 4 & discarded & early & - & Trunc. & -132 \\
& MI300A, MI300X & (2,24) & 4 & subnormal & late & (24,31,RD) & RNE. & -126 \\
\bottomrule
\end{tabular}
}

\vspace{2mm}

{\footnotesize
\textbf{Note:} $(24,31,\mathrm{RD})$ indicates that RD is applied beyond the 24th fractional bit when $c$ is shifted, and beyond the 31st fractional bit when the product sum $s_{p_i,\mathrm{sum}}$ is shifted. * indicates the mixed use of RD and RZ, as described in Algorithm~\ref{alg:cdna3_fp8}. $\mathrm{odd\text{-}even}$ denotes the interleaved product-addition pattern, where odd- and even-indexed products are accumulated separately. MI210 and MI250 GPUs support FP16/BF16 and implement SFMA with the grouping shown in Fig.~\ref{fig:CDNA2}. 
The output is assumed to be in fp32 format.
 
}

\end{minipage}
}

\end{center}
